Lower Bounds for Unambiguous Automata via Communication Complexity

We use results from communication complexity, both new and old ones, to prove lower bounds for unambiguous finite automata (UFAs). We show three results. $\textit{Complement:}$ There is a language $L$ recognised by an $n$-state UFA such that the complement language $\overline{L}$ requires NFAs with $n^{\tilde{\Omega}(\log n)}$ states. This improves on a lower bound by Raskin. $\textit{Union:}$ There are languages $L_1$, $L_2$ recognised by $n$-state UFAs such that the union $L_1\cup L_2$ requires UFAs with $n^{\tilde{\Omega}(\log n)}$ states. $\textit{Separation:}$ There is a language $L$ such that both $L$ and $\overline{L}$ are recognised by $n$-state NFAs but such that $L$ requires UFAs with $n^{\Omega(\log n)}$ states. This refutes a conjecture by Colcombet.

==> parts/conclusions.tex <==
\section{Conclusions}
In the main results, \cref{thm:complement,thm:separation}, we have obtained super-polynomial but quasi-polynomial lower bounds on UFA complementation and separation.
These bounds are not known to be tight; indeed, in both cases the best known upper bound is exponential.
At the same time, we have transferred techniques from communication complexity relatively directly.
More concretely, both main theorems hinge on a finite language $\{x y \mid F(x,y) = 1\}$ where $F$ is a two-party function whose communication complexity is in a sense extreme.
This suggests two kinds of opportunities for future work:
\begin{itemize}
\item Can other techniques from communication complexity improve the lower bounds further? Perhaps by somehow iterating a two-party function or via multi-party communication complexity?
\item Can techniques for proving upper bounds on communication complexity be adapted to prove upper bounds on the size of automata?
\end{itemize}
